VisEscape: A Benchmark for Evaluating Exploration-driven Decision-making in Virtual Escape Rooms

Escape rooms present a unique cognitive challenge that demands exploration-driven planning: with the sole instruction to 'escape the room', players must actively search their environment, collecting information, and finding solutions through repeated trial and error. Motivated by this, we introduce VisEscape, a benchmark of 20 virtual escape rooms specifically designed to evaluate AI models under these challenging conditions, where success depends not only on solving isolated puzzles but also on iteratively constructing and refining spatial-temporal knowledge of a dynamically changing environment. On VisEscape, we observe that even state-of-the-art multi-modal models generally fail to escape the rooms, showing considerable variation in their progress and problem-solving approaches. We find that integrating memory management and reasoning contributes to efficient exploration and enables successive hypothesis formulation and testing, thereby leading to significant improvements in dynamic and exploration-driven environments

==> figs/memory.tex <==
\begin{figure}[!htbp]
\centering
\includegraphics[width=\linewidth]{imgs/memory.png}
\caption{\todo{how about iteration in figure?}}
\label{fig:memory}
\end{figure}


==> tables/data_stat.tex <==
\begin{table}[htbp]
    \centering
    \scriptsize
    \resizebox{\linewidth}{!}{    
    \begin{tabular}{c|ccccc}
    \toprule
    &Scene &Receptacle &Item &Quiz &Interaction \\
    \midrule
    \# Total &1084 &118 &102 &27 &311 \\
    \midrule
    \# Types &662 &32 &23 &27 &37 \\
    \midrule
    Avg./room &54.2 &5.9 &5.1 &1.4 &15.6 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Statistics for scenes, receptacles, items, quizzes, and interactions in \datasetname.}
    \label{tab:data_stat}
\end{table}


==> tables/memory_ablation_short.tex <==
\begin{table}[h]\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule

\textbf{Model}& \textbf{Memory} & \textbf{SR$\uparrow$(\%)} & \textbf{GC$\uparrow$(\%)} & \textbf{HCR$\downarrow$(\%)} & \textbf{SPL$\uparrow$(\%)} & \textbf{Step$\downarrow$} \\
\midrule
\multirow{2}{*}{InternVL2.5-38B} & O & 66.7 & 79.2 & 41.7 & 12.2 & 210.5 \\
& X & 10.0 & 59.2 & 41.9 & 1.6 & 287.0 \\
\midrule
\multirow{2}{*}{LLaVA-v1.6-34B} & O & 15.0 & 34.8 & 65.0 & 1.5 & 289.8 \\
& X & 0.0 & 15.2 & 55.2 & 0.0 & 300.0 \\
\bottomrule
\end{tabular}
}
\caption{Ablation results in \exphint~comparing performance in the presence and absence of memory modules. The scores of all metrics decrease significantly when memory modules is absent.}
\label{tab:no_memory_short}
\end{table}


==> tables/react_vs_act.tex <==
\begin{table}[!htp]\centering
\scriptsize
\begingroup
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccc}\toprule
\multirow{2}{*}{Model} &\multirow{2}{*}{\react= \act} &\multicolumn{3}{c}{\react $\neq$ \act} \\\cmidrule{3-5}
& & \react > \act & \react < \act &\textit{ambig.} \\\midrule


Claude 3.5 Sonnet &0.47 &0.5 &0.1 &0.4 \\
GPT-4o & 0.54 &0.1 &0.4 &0.4\\
Gemini-1.5-Pro &0.52 &0.5 &0.1 &0.4 \\
GPT-4o-mini & 0.53 &0.1 &0.4 &0.4\\
\bottomrule
\end{tabular}
}
\caption{Generated by Spread-LaTeX}\label{tab: }

\endgroup %
\end{table}

